Annotating sleep states in children from wrist-worn accelerometer data using Machine Learning

Sleep detection and annotation are crucial for researchers to understand sleep patterns, especially in children. With modern wrist-worn watches comprising built-in accelerometers, sleep logs can be collected. However, the annotation of these logs into distinct sleep events: onset and wakeup, proves to be challenging. These annotations must be automated, precise, and scalable. We propose to model the accelerometer data using different machine learning (ML) techniques such as support vectors, boosting, ensemble methods, and more complex approaches involving LSTMs and Region-based CNNs. Later, we aim to evaluate these approaches using the Event Detection Average Precision (EDAP) score (similar to the IOU metric) to eventually compare the predictive power and model performance.

==> chapters/8_work_split.tex <==
\section{Work Split}

The authors contributions to the project are as follows.

\textbf{Ashwin Ram} and \textbf{Zizhe Jiang} worked on Related Work (\ref{sec:related_work}), Methodology (\ref{sec:methodology}), Metrics \& Evaluation (\ref{sec:metrics}), and Results (\ref{sec:results}).

\textbf{Shuvam Keshari} and \textbf{Sundar Sripada V. S.} worked on the rest of Introduction (\ref{sec:intro}), Problem Description (\ref{sec:problem_description}), and the Abstract. 
